Intersection Numbers, Polynomial Division and Relative Cohomology

We present a simplification of the recursive algorithm for the evaluation of intersection numbers for differential $n$-forms, by combining the advantages emerging from the choice of delta-forms as generators of relative twisted cohomology groups and the polynomial division technique, recently proposed in the literature. We show that delta-forms capture the leading behaviour of the intersection numbers in presence of evanescent analytic regulators, whose use is, therefore, bypassed. This simplified algorithm is applied to derive the complete decomposition of two-loop planar and non-planar Feynman integrals in terms of a master integral basis. More generally, it can be applied to derive relations among twisted period integrals, relevant for physics and mathematical studies.

==> ex_pentabox.tex <==
\subsection{Pentabox}

\label{subsec:pentabox}
\begin{figure}[H]
\centering
\includegraphics[width=0.9\textwidth]{figures/penta_fig_2.pdf}
\caption{The 47 sectors of the pentabox family that contain master integrals. When there are $n > 1$ MIs in a sector, that is indicated as $\mathcal{S}_i \times n$.
    \label{fig:pentaboxsectors}
}
\end{figure}
The integral family of the pentabox is given in terms of
\begin{align}
z_1 &= k_1^2, & z_2 &= (k_1{-}p_1)^2, & z_3 &= (k_1{-}p_1{-}p_2)^2, & z_4 &= (k_2{-}p_1{-}p_2)^2,\nonumber \\
z_5 &= (k_2{-}p_1{-}p_2{-}p_3)^2, & z_6 &= (k_2{+}p_5)^2, & z_7 &= (k_2)^2, & z_8 &= (k_1{-}k_2)^2,\nonumber\\
z_9 &= (k_2{-}p_1)^2, & z_{10} &= (k_1{-}p_1{-}p_2{-}p_3)^2, & z_{11} &= (k_1{+}p_5)^2 , 
\end{align}
where $z_9, \ z_{10}, \ z_{11}$ are irreducible scalar products. The kinematics is such that:
\begin{align}
    p_i^2 &  =  0 , &  s_{12} & =  (p_1{+}p_2)^2 , & s_{23} & =  (p_2{+}p_3)^2 ,  \nonumber \\  s_{34} & =  (p_3{+}p_4)^2, 
   &  s_{45}  & = (p_4{+}p_5)^2 , & s_{51} & = ( p_5 + p_1 )^2\ . 
\end{align}
This integral family has (before the application of symmetry relations) 62
master integrals, which belong to 47 sectors, depicted in \figref{fig:pentaboxsectors}.
We are interested in decomposing the target integral:
\begin{equation}
    I  \ = \ \int \ d\mathbf{z} \  u(\mathbf{z}) \frac{z_9^2}{z_1z_2z_3z_4z_5z_6z_7 z_8}
\end{equation}
in terms of master integrals via a complete set of spanning cuts, as:
\begin{equation}
    I \ = \ \sum_{i=1}^{62} c_i \ J_i\ . 
\end{equation}

The set of spanning cuts is given by the cuts corresponding to the maximal cuts of the first ten topologies $\mathcal{S}_1-\mathcal{S}_{10}$, and we will now go through them one by one.

